Visconde: Multi-document QA with GPT-3 and Neural Reranking

This paper proposes a question-answering system that can answer questions whose supporting evidence is spread over multiple (potentially long) documents. The system, called Visconde, uses a three-step pipeline to perform the task: decompose, retrieve, and aggregate. The first step decomposes the question into simpler questions using a few-shot large language model (LLM). Then, a state-of-the-art search engine is used to retrieve candidate passages from a large collection for each decomposed question. In the final step, we use the LLM in a few-shot setting to aggregate the contents of the passages into the final answer. The system is evaluated on three datasets: IIRC, Qasper, and StrategyQA. Results suggest that current retrievers are the main bottleneck and that readers are already performing at the human level as long as relevant passages are provided. The system is also shown to be more effective when the model is induced to give explanations before answering a question. Code is available at \url{https://github.com/neuralmind-ai/visconde}.

==> tables/IIRC.tex <==

\begin{table}[t]
\centering
\caption{IIRC results considering the links (L) related to the documents and ground truth contexts (C). ``Gold Ctx'' refers to using ground truth contexts as input to the aggregator module. LongT5 numbers were taken from the SCROLLS~\cite{shaham2022scrolls} leaderboard.}
\label{tab:iirc_results}
\begin{tabular}{lcccc}
\toprule
\textbf{Model} & \textbf{Gold Ctx} & \textbf{CoT}                                   & \textbf{F1}    & \textbf{EM}    \\ \midrule
Human         & - & -                            & 88.4 & 85.7 \\
Ferguson et al.~\cite{ferguson-etal-2020-iirc} & - &    &  31.1 & 27.7  \\
Ferguson et al.~\cite{ferguson-etal-2020-iirc} L & - &    & 32.5 & 29.0  \\
Ferguson et al.~\cite{ferguson-etal-2020-iirc} & \checkmark & -  & 70.3 & 65.6 \\

\midrule
Visconde & \checkmark & \checkmark & 84.2 & 74.7 \\
Visconde  & \checkmark & -   & 80.3 & 70.0 \\
%Visconde (4-shot, dyn prompt, \textbf{w/o CoT}) L + C & Oracle & - & 671 & 573 \\
Visconde L & - & \checkmark   & 50.2 & 43.3 \\
Visconde L & - & -    & 48.2 & 40.7 \\
Visconde & - & \checkmark & 47.9 & 40 \\
Visconde (static prompt) L & \checkmark & - & 74.3 & 62.7 \\
\bottomrule
\end{tabular}
\end{table}

==> tables/qasper.tex <==
\begin{table}[]
\centering
\footnotesize
\caption{Qasper results.}
\label{tab:qasper_results}
\begin{tabular}{@{}p{3cm}cccccc@{}}
\toprule
Model                               & Extractive & Abstractive & Boolean & None  & Evidence F1 & Answer F1 \\ \midrule
Human                               & 58.9      & 39.7       & 79.0   & 69.4 & 71.6       & 60.9     \\
\midrule
\textit{Supervised}\\
LED-base                            & 30.0      & 15.0       & 68.9   & 45.0 & 29.9       & 33.6     \\
MoD  \cite{ray2022mod}                               &        -    &     -        &     -    &   -    &      -       & 37.6     \\
BART-LS~\cite{xiong2022adapting} & - & - & - & - & - & 48.7\\
LongT5~\cite{xiong2022longt5} & - & - & - & - & - & 53.1\\
\midrule
\textit{Few-shot}\\
% MultiDocQA (3-shot, dynamic prompt) & 57.0      & 43.3       & 85.7   & 45.5 & 51.8       & 57.5     \\
Visconde (3-shot, static)         & 52.3      & 21.7      & 86.2       & 48.3 & 38.5    & 49.1 \\
\bottomrule
\end{tabular}
\end{table}

==> tables/results_all.tex <==
\begin{table}[th!]
\footnotesize
\centering
\caption{Visconde and similar approaches results on IIRC, Qasper and StrategyQA.}
\label{tab:results}
\begin{tabular}{lcccc}
\toprule
\multicolumn{5}{c}{\textbf{IIRC}} \\ \midrule
Model                                  & \multicolumn{2}{c}{F1}            & \multicolumn{2}{c}{EM}            \\ \midrule
Human                                  & \multicolumn{2}{c}{88.4}          & \multicolumn{2}{c}{85.7}          \\
\midrule
\textit{Finetuned}\\
Ferguson et al.~\cite{ferguson-etal-2020-iirc}   & \multicolumn{2}{c}{31.1}          & \multicolumn{2}{c}{27.7}          \\
Ferguson et al.~\cite{ferguson-etal-2020-iirc} Linked pages & \multicolumn{2}{c}{32.5}          & \multicolumn{2}{c}{29.0}          \\
Ferguson et al.~\cite{ferguson-etal-2020-iirc} Gold Ctx   & \multicolumn{2}{c}{70.3}          & \multicolumn{2}{c}{65.6}          \\
PReasM (pretrain + finetuning) \cite{trivedi2022teching} Gold Ctx & \multicolumn{2}{c}{-} & \multicolumn{2}{c}{73.3} \\
PReasM (pretrain + finetuning) \cite{trivedi2022teching} & \multicolumn{2}{c}{-} & \multicolumn{2}{c}{47.2} \\
Sup$_{A+QA}$ (supervised) \cite{ferguson-etal-2022-retrieval}  & \multicolumn{2}{c}{51.6} & \multicolumn{2}{c}{-}
\\
\midrule
\textit{Few-shot}\\
Visconde (4-shot dynamic prompt)  Gold Ctx and CoT                                                              & \multicolumn{2}{c}{84.2}          & \multicolumn{2}{c}{74.7}          \\
Visconde (4-shot dynamic prompt) Gold Ctx & \multicolumn{2}{c}{80.3}          & \multicolumn{2}{c}{70.0}          \\
Visconde (4-shot static prompt) Gold Ctx                                         & \multicolumn{2}{c}{74.3}          & \multicolumn{2}{c}{62.7}          \\
% Visconde (4-shot dynamic prompt) L                                                             & -                         & \checkmark & 50.2          & 43.3          \\
Visconde (4-shot dynamic prompt) Linked pages      & \multicolumn{2}{c}{48.2}          & \multicolumn{2}{c}{40.7}          \\
Visconde (4-shot dynamic prompt) CoT   & \multicolumn{2}{c}{47.9}          & \multicolumn{2}{c}{40.0}            \\
\toprule
\multicolumn{5}{c}{\textbf{QASPER}}                                                                                                                                     \\\midrule
Model                                                                  & \multicolumn{2}{c}{Evidence F1}                       & \multicolumn{2}{c}{Answer F1} \\ \midrule
Human                                                                  & \multicolumn{2}{c}{71.6}                              & \multicolumn{2}{c}{60.9}      \\
LED-base                                                               & \multicolumn{2}{c}{29.9}                              & \multicolumn{2}{c}{33.6}      \\
% MoD \cite{ray2022mod}                                 & \multicolumn{2}{c}{-}                                 & \multicolumn{2}{c}{37.6}      \\
% BART-LS~\cite{xiong2022longt5}                 & \multicolumn{2}{c}{-}                                 & \multicolumn{2}{c}{48.7}      \\
SOTA~\cite{xiong2022longt5}                    & \multicolumn{2}{c}{-}                                 & \multicolumn{2}{c}{53.1}      \\
Visconde (3-shot, static prompt)                                              & \multicolumn{2}{c}{38.5}                              & \multicolumn{2}{c}{49.1}      \\
\toprule
\multicolumn{5}{c}{\textbf{StrategyQA}}                                                                                                                                 \\ \midrule
Model                                                                  & Acc                       & Recall@10                 & \multicolumn{2}{c}{SARI}      \\ \midrule
Human                                                                  & 87.00                     & 0.586                       & \multicolumn{2}{c}{}          \\
Baseline                                                               & 63.60                     & 0.195                       & \multicolumn{2}{c}{}          \\
Leaderboard's SOTA                                                                   & 69.80                     & 0.537                       & \multicolumn{2}{c}{0.555}       \\
GOPHER-280B OB$^{PoE}_{Google}$ \cite{lazaridou2022internet} & 66.20 & - & \multicolumn{2}{c}{-} 
\\
Visconde (1-shot, static prompt, gold evidences)                       & 73.80                     & -                         & \multicolumn{2}{c}{-}         \\
Visconde (1-shot, static prompt)                                       & 69.43                     & 0.331                       & \multicolumn{2}{c}{0.570}       \\
% Visconde (1-shot, dynamic prompt)                                      & 63.32                     & 0.331                       & \multicolumn{2}{c}{0.570}      \\ 
\bottomrule
\end{tabular}
\end{table}

==> tables/strategyQA.tex <==
\begin{table}[]
\centering

\caption{StrategyQA results.}
\label{tab:strategyqa_results}
\begin{tabular}{@{}lccc@{}}
\toprule
Model                                               & Acc     & Recall@10 & SARI  \\ \midrule
Human                                               & 87.00 & 0.586     &       \\
Baseline                                            & 63.60 & 0.195     &       \\
SOTA \cite{}                                                & 69.80 & 0.537     & 0.555 \\
\midrule
\textit{Few-shot}\\
Visconde (1-shot, static prompt, gold evidences)  & 73.80 & -         & -     \\
Visconde (1-shot, static prompt)                  & 69.43 & 0.331     & 0.570 \\
Visconde (1-shot, dynamic prompt)                 & 63.32 & 0.331     & 0.570 \\ \bottomrule
\end{tabular}
\end{table}
